WoLF: Wide-scope Large Language Model Framework for CXR Understanding

Significant methodological strides have been made toward Chest X-ray (CXR) understanding via modern vision-language models (VLMs), demonstrating impressive Visual Question Answering (VQA) and CXR report generation abilities. However, existing CXR understanding frameworks still possess several procedural caveats. (1) Previous methods solely use CXR reports, which are insufficient for comprehensive Visual Question Answering (VQA), especially when additional health-related data like medication history and prior diagnoses are needed. (2) Previous methods use raw CXR reports, which are often arbitrarily structured. While modern language models can understand various text formats, restructuring reports for clearer, organized anatomy-based information could enhance their usefulness. (3) Current evaluation methods for CXR-VQA primarily emphasize linguistic correctness, lacking the capability to offer nuanced assessments of the generated answers. In this work, to address the aforementioned caveats, we introduce WoLF, a Wide-scope Large Language Model Framework for CXR understanding. To resolve (1), we capture multi-faceted records of patients, which are utilized for accurate diagnoses in real-world clinical scenarios. Specifically, we adopt the Electronic Health Records (EHR) to generate instruction-following data suited for CXR understanding. Regarding (2), we enhance report generation performance by decoupling knowledge in CXR reports based on anatomical structure even within the attention step via masked attention. To address (3), we introduce an AI-evaluation protocol optimized for assessing the capabilities of LLM. Through extensive experimental validations, WoLF demonstrates superior performance over other models on MIMIC-CXR in the AI-evaluation arena about VQA (up to +9.47%p mean score) and by metrics about report generation (+7.3%p BLEU-1).

==> subtex/3-2_exp-table-b.tex <==
\renewcommand{\arraystretch}{1.0}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\begin{table}[!ht]
    \begin{center}
    \caption{Accuracy of the CXR-VQA task by topic. We utilize the ELIXR~\cite{elixr} framework for assessing this VQA performance.}
    { \footnotesize
    \scalebox{0.95}{
    \begin{tabular}{ c | c | c c c } \toprule
     \textbf{Accuracy} $\uparrow$ & \textbf{All} & \textbf{Presence} & \textbf{Location} & \textbf{Size, severity, type} \\ \midrule
    ELIXR~\cite{elixr}\* & 54.8\% & 64.5\% & 41.0\% & 25.0\% \\
    XrayGPT~\cite{xraygpt} & 25.2\% & 27.4\% & 21.9\% & 20.3\% \\
    LLM-CXR~\cite{llmcxr} & 56.7\% & 60.1\% & 49.0\% & 53.1\% \\
    MedXChat~\cite{medxchat} & 61.2\% & 61.5\% & 56.3\% & 68.8\% \\ \midrule
    \rowcolor{LightCyan!40}
    \shortname{} & \textbf{62.1}\% & \textbf{67.9}\% & \textbf{56.9}\% & \textbf{71.8}\% \\ 
    \bottomrule
    \end{tabular}
    }
    }
\end{center}
\end{table}

==> subtex/3-3_exp-table-c.tex <==
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\begin{table}[!th]
\begin{center}
\caption{VQA-RAD. dagger : fine-tuned with VQA-RAD Med-VInT, ELIXR Experiments mentioned on~\cite{elixr}}
{ \footnotesize
\scalebox{0.9}{\begin{tabular}{ c | c | c c c} \toprule
 \textbf{Accuracy} $\uparrow$ & \textbf{Fine-tuning\textsuperscript{\textdagger}} & \textbf{Both} & \textbf{Open} & \textbf{Closed} \\ \midrule
Med-VInT~\cite{med-vint} & \faCheck & \textbf{81.6}\% & \textbf{86.8}\% & \textbf{73.7}\% \\
\midrule
Med-VInT~\cite{med-vint} & \faTimes & 27.9\% & 28.2\% & 27.1\% \\
ELIXR~\cite{elixr} & \faTimes & 58.7\% & 69.3\% & 37.9\% \\
\bottomrule
\rowcolor{LightCyan!40}
WoLF & \faTimes & \textbf{77.9}\% & \textbf{82.7}\% & \textbf{57.2}\% \\ \bottomrule
\end{tabular}
}
\label{vqa-rad}
}
\end{center}
\end{table}

==> subtex/3-4-2_exp-table2-aif-winrate.tex <==
\begin{table}[!h]
\setlength{\belowrulesep}{0pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{Win-rate for each comparable model.}
\scalebox{0.76}{\begin{tabular}{c|cc|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\bf Comparison} & \bf \multicolumn{2}{l}{\bf Accuracy} & \bf \multicolumn{2}{l}{\bf Helpfulness} & \bf \multicolumn{2}{l}{\bf Relevance} & \bf \multicolumn{2}{l}{\bf Hallucination} & \bf \multicolumn{2}{l}{\bf Universal}  \\ 
\cmidrule[.55pt]{2-11}
 & Gemini & PaLM-2 & Gemini & PaLM-2& Gemini & PaLM-2& Gemini & PaLM-2& Gemini & PaLM-2  \\ 
\midrule
\textbf{\shortname{}} vs. LLaVA-Med~\cite{llmcxr} & 71.50\% &00.00\%& 77.75\% &00.00\%& 76.25\% &00.00\%& 84.25\% &00.00\%& 73.40\%&00.00\%  \\ 
\textbf{\shortname{}} vs. LLM-CXR~\cite{llava-med} & 75.80\% &00.00\%& 83.68\% &00.00\%& 81.05\% &00.00\%& 84.23\% &00.00\%& 77.68\% &00.00\%  \\ 
\textbf{\shortname{}} vs XrayGPT~\cite{xraygpt} & 83.30\% &00.00\%& 86.15\% &00.00\%& 83.80\% &00.00\%& 87.05\% &00.00\%& 84.63\%&00.00\%\\ 
\textbf{\shortname{}} vs. \textbf{\shortname{}$^\dagger$} & 56.40\% &00.00\%& 53.80\% &00.00\%& 53.81\% &00.00\%& 68.73\% &00.00\%& 55.20\%&00.00\%\\ 
\textbf{\shortname{}} vs.\textbf{\shortname{}$^\ddagger$} & 47.20\% &00.00\%& 46.70\% &00.00\%& 47.05\% &00.00\%& 49.95\% &00.00\%& 48.80\%&00.00\%\\ 
\bottomrule
\end{tabular}}
\label{win-rate}
\end{center}
\end{table}

==> subtex/3-5_exp-qualitative.tex <==
qualitative results

==> subtex/3-6_exp-prompts.tex <==
prompts while AI-evaluation

==> subtex/3-7_setup.tex <==
\textbf{\textit{Training Details}} \texttt{Vicuna-7b}~\cite{vicuna} is used for core LLM with LoRA~\cite{lora} fine-tuning. CLIP-ViT-L-14~\cite{clip} is used as a frozen image encoder during training. The batch size is set to 64. The learning rate is set at $2\text{e-}5$, and the training for each stage was conducted over 2 epochs.

==> subtex/supp_a1.tex <==
\begin{table}[!h]
\setlength{\belowrulesep}{0pt}
\setlength{\aboverulesep}{0pt}
\centering
\caption{Ablation study of main paper Table~\ref{tab1}.
$^-$ for a given set of \shortname{} trained without EHRXQA~\cite{ehrxqa}. $^+$ for a given set of \shortname{} given corresponding patient EHR while inference.}
\scalebox{0.80}{
\begin{tabular}{c|cccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{\includegraphics[height=1em]{pic/gemini.png}Gemini~\cite{gemini}} \\
& \textbf{Accuracy} & \textbf{Helpfulness} & \textbf{Relevance} & \textbf{Hallucination} & \textbf{Universal} & \textbf{Mean} \\
\midrule
\rowcolor{LightCyan!40}
\shortname{}$^-$ & 71.58\scriptsize($\pm$0.77) & 72.10\scriptsize($\pm$0.51) & 69.27\scriptsize($\pm$1.09) & 78.14\scriptsize($\pm$2.13) & 74.96\scriptsize($\pm$0.77) & \multicolumn{1}{|c}{73.21\scriptsize($\pm$0.12)} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{LightCyan!40}
\shortname{} & \underline{73.03}\scriptsize($\pm$0.64) & \underline{73.19}\scriptsize($\pm$0.87) & \underline{72.34}\scriptsize($\pm$0.42) & \underline{79.02}\scriptsize($\pm$0.67) & \underline{75.95}\scriptsize($\pm$0.49) & \multicolumn{1}{|c}{\underline{74.70}\scriptsize($\pm$0.34)} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{LightCyan!40}
\shortname{}$^+$ & \textbf{77.80}\scriptsize($\pm$0.24) & \textbf{74.55}\scriptsize($\pm$0.53) & \textbf{73.03}\scriptsize($\pm$0.63) & \textbf{82.49}\scriptsize($\pm$0.83) & \textbf{77.73}\scriptsize($\pm$0.43) & \multicolumn{1}{|c}{\textbf{77.12}\scriptsize($\pm$0.16)} \\
\toprule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \multicolumn{5}{c}{\includegraphics[height=1em]{pic/PaLM2.png}PaLM-2~\cite{palm2}} \\
& \textbf{Accuracy} & \textbf{Helpfulness} & \textbf{Relevance} & \textbf{Hallucination} & \textbf{Universal} & \textbf{Mean}\\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{LightCyan!40}
\shortname{}$^-$ & 77.51\scriptsize($\pm$0.98) & 76.77\scriptsize($\pm$1.36) & 74.42\scriptsize($\pm$2.75) & 81.93\scriptsize($\pm$1.19) & 77.45\scriptsize($\pm$2.60) & \multicolumn{1}{|c}{77.61\scriptsize($\pm$1.26)} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{LightCyan!40}
\shortname{} & \underline{79.54}\scriptsize($\pm$0.77) & \underline{79.93}\scriptsize($\pm$1.22) & \textbf{79.21}\scriptsize($\pm$0.58) & \underline{85.30}\scriptsize($\pm$3.74) & \underline{78.18}\scriptsize($\pm$0.91) & \multicolumn{1}{|c}{\underline{80.13}\scriptsize($\pm$1.17)}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rowcolor{LightCyan!40}
\shortname{}$^+$ & \textbf{81.09}\scriptsize($\pm$0.30) & \textbf{81.60}\scriptsize($\pm$1.56) & \underline{79.20}\scriptsize($\pm$0.55) & \textbf{86.22}\scriptsize($\pm$3.62) & \textbf{78.84}\scriptsize($\pm$1.89) & \multicolumn{1}{|c}{\textbf{81.39}\scriptsize($\pm$1.65)} \\
\bottomrule
\end{tabular}
}
\label{tab1}
\end{table}


==> subtex/supp_a2.tex <==
\begin{table}[!h]
\setlength{\belowrulesep}{0pt}
\setlength{\aboverulesep}{0pt}
\begin{center}
\caption{Win-rate for each comparable model. The win-rate of model X versus model Y is obtained by counting how many times the responses of model X beat Y. For instance, a \textbf{50\%} signifies X beats Y in half of the Questions, while Y beats X in the remaining half.}
\scalebox{0.76}{\begin{tabular}{c|cg|cg|cg|cg|cg}
\toprule
\multirow{2}{*}{\bf Comparison} & \bf \multicolumn{2}{l}{\bf Accuracy} & \bf \multicolumn{2}{l}{\bf Helpfulness} & \bf \multicolumn{2}{l}{\bf Relevance} & \bf \multicolumn{2}{l}{\bf Hallucination} & \bf \multicolumn{2}{l}{\bf Universal}  \\ 
\cmidrule[.55pt]{2-11}
 & Gemini & PaLM-2 & Gemini & PaLM-2& Gemini & PaLM-2& Gemini & PaLM-2& Gemini & PaLM-2  \\ 
\midrule
\textbf{\shortname{}} vs. LLaVA-Med~\cite{llmcxr} & 71.50\% &72.13\%& 77.75\% &77.90\%& 76.25\% &76.78\%& 84.25\% &84.85\%& 73.40\%&73.70\%  \\ 
\textbf{\shortname{}} vs. LLM-CXR~\cite{llava-med} & 64.05\% &61.50\%& 61.73\% &61.58\%& 61.95\% &61.58\%& 63.93\% &64.18\%& 63.6\% &63.45\%  \\ 
\textbf{\shortname{}} vs. XrayGPT~\cite{xraygpt} & 75.80\% &75.83\%& 83.68\% &83.15\%& 81.05\% &82.05\%& 84.23\% &84.68\%& 84.93\%&84.63\%\\ 
\textbf{\shortname{}} vs. \textbf{\shortname{}$^\dagger$} & 56.40\% &57.10\%& 53.80\% &54.50\%& 53.81\% &54.00\%& 68.73\% &68.80\%& 55.20\%&55.40\%\\ 
\textbf{\shortname{}} vs.\textbf{\shortname{}$^\ddagger$} & 47.20\% &47.45\%& 46.70\% &47.12\%& 47.05\% &47.95\%& 49.90\% &49.95\%& 48.80\%&49.20\%\\ 
\bottomrule
\end{tabular}}
\label{win-rate}
\end{center}
\end{table}

==> subtex/supp_c.tex <==
\begin{figure}[!h]
\centering
    \includegraphics[width=\textwidth]{figures/fig_prompt.pdf}
    \caption{Evaluation Prompt for scoring and ranking.}
    \label{supp_fig1}
\end{figure}


==> subtex/supp_d.tex <==
\begin{figure}[h]
    \centering
    \scalebox{0.86}{
    \begin{tabular}{c}
        \includegraphics[width=\textwidth]{figures/fig_qualitative.pdf}
        
    \end{tabular}
    }
    \caption{Qualitative results of visual question-answering scenarios. In (a) and (b), we feed models with patient histories and medication details from EHRs. WoLF utilizes this to deliver more accurate responses.}\
    \label{tab:my_label}
\end{figure}
